EXPRESS: An LLM-Generated Explainable Property Valuation System with Neighbor Imputation

The demand for property valuation has attracted significant attention from sellers, buyers, and customers applying for loans. Reviews of existing approaches have revealed shortcomings in terms of not being able to handle missing value situations, as well as lacking interpretability, which means they cannot be used in real-world applications. To address these challenges, we propose an LLM-Generated EXplainable PRopErty valuation SyStem with neighbor imputation called EXPRESS, which provides the customizable missing value imputation technique, and addresses the opaqueness of prediction by providing the feature-wise explanation generated by LLM. The dynamic nearest neighbor search finds similar properties depending on different application scenarios by property configuration set by users (e.g., house age as criteria for the house in rural areas, and locations for buildings in urban areas). Motivated by the human appraisal procedure, we generate feature-wise explanations to provide users with a more intuitive understanding of the prediction results.

==> Section/3-Experiment.tex <==
\section{Experiment} 
% MAPE equation
% data statistic
% Prediction performance (random forests, neural networks)
% \subsection{K Value Ablation}
% In order to validate the optimal k value in the nearest neighbor search, we conduct an ablation study to investigate the impact of the k value in Figure \ref{fig:k}.
% Considering the inference time constraints for the online system, this experiment was restricted to the range between k=0 and k=30.
% No optimal k is identified across different property types (i.e. Building, Apartment, House).
% Therefore, we designed the dynamic nearest neighbor search to calculate the best k based on the number of neighbor properties for every instance.
In the experiment, since different property types have distinct characteristics, we separated properties into three types, Building, Apartment, and House, and trained separate models for each property type.
We adopted the mean absolute percentage error (MAPE) as the evaluation metric to measure the prediction results.

\subsection{Imputation Ablation}
Table \ref{tab:imputation} presents the performance of various imputation techniques, including our proposed neighbor imputation, no imputation, and average imputation. 
The results indicate the superiority of our proposed imputation method over others. 
The differences between our method and the ideal situation range from approximately 9\% to 25\%.


% \begin{figure}
%   \par\bigskip
%   \centering
%   \begin{subfigure}{0.15\textwidth}
%           \centering
%           \includegraphics[width=\linewidth]{Figure/k_building.png}
%           \caption{Building}
%           \label{fig:Building}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.15\textwidth}
%           \centering
%           \includegraphics[width=\linewidth]{Figure/k_apartment.png}
%           \caption{Apartment}
%           \label{fig:Apartment}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.15\textwidth}
%           \centering
%           \includegraphics[width=\linewidth]{Figure/k_house.png}
%           \caption{House}
%           \label{fig:House}
%   \end{subfigure}
%   \caption{The ablation studies of k values.} \label{fig:k}
% \end{figure}

\begin{table}
\begin{center}
    \caption{MAPE ($\downarrow$) performance of different imputation techniques. "No Imputation" refers to utilizing only a few features input by users without any imputation. "Average Imputation" involves imputing the mean value of all the data. The ideal situation represents the upper bound of performance, indicating the scenario where all features are available.}
    \input{Table/imputation} \label{tab:imputation}
\end{center}
\end{table}

==> Section/4-Use-Cases.tex <==
\section{Demonstration} \label{Demonstration}
\begin{figure}
  \centering
  \par\bigskip
  \begin{subfigure}{0.5\textwidth}
          \centering
          \includegraphics[width=\linewidth]{Figure/configuration.png}
          \caption{The interface of Property Configuration.}
          \label{fig:platform-1}
  \end{subfigure}
  \par\bigskip
  \begin{subfigure}{0.5\textwidth}
          \centering
          \includegraphics[width=\linewidth]{Figure/result.png}
          \caption{The interface of Prediction Result.}
          \label{fig:platform-2}
  \hfill
  \end{subfigure}
  \caption{System interface of EXPRESS.}
\end{figure}

EXPRESS is a fully open-source system that utilizes Flask which is a Python framework for its back-end logic, and React as a Javascript front-end framework for its user interface.
Additionally, we utilized the Geoencoding API provided by Google to display the spatial relation between the input property and the selected neighboring properties.


\subsection{System Procedures}
The basic procedures are as follows: Select the property type and enter property details.$\,\to\,$Enter the property configurations.$\,\to\,$View the valuation result, pairwise explanation, and visualization on the map.$\,\to\,$Verify the result using the LLM-generated explanation and the spatial relationships shown on the map.
It basically consists of two interfaces: property configuration and prediction result, which consists of predicted price, pair-wise explanation, textual explanation, and the spatial relationship shown on the map.
More details about these two interfaces are as follows:

\textbf{Property Configuration.} 
% \subsection{Property Configuration}
As illustrated in Figure \ref{fig:platform-1}, users initiate the process by selecting the property type and entering details, such as address, house age, total floors, and parking areas.
Following this, the property configuration enables users to set neighboring conditions for identifying appropriate neighbors.
In cases where users lack specific criteria for their target property, they can input a few conditions or leave the fields entirely blank.
% If the system detects an insufficient number of neighbors, it will automatically revert to the default configuration to mitigate potential biases stemming from a limited number of properties.

\textbf{Prediction Result.} 
% \subsection{Prediction Result}
After entering all the information, the system will automatically impute all the missing values of required features and generate the prediction result as shown in Figure \ref{fig:platform-2}.
On the left-hand side, a map illustrates the location of the target property indicated by a red icon, alongside its neighboring properties denoted by blue icons. 
On the right-hand side, the imputation result and predicted unit price are displayed at the top, while all neighboring properties are listed below.
Users can make their own judgments based on the pairwise explanation.

\subsection{Use Cases Studies}
First, we demonstrate the practical utilization of the prediction result and pairwise explanation.
As depicted in Figure \ref{fig:case-2}, let us consider an apartment located in Taipei as an example.
The predicted unit price is about 30 thousand NTD per square meter, and users can scroll through the rows to view all the imputation values.
Below are neighboring properties to the given apartment; among the six cases showcased, two properties are older than the target apartment, two are approximately the same age, and two are younger.
In property valuation, there typically exists a negative correlation between house age and unit price.
The data presented in this case aligns with this domain understanding.
Users are encouraged to employ their own knowledge and expertise to interpret these results.
Due to space limitations, we cannot show all the neighbors and all the reasons.

On the other hand, considering the diversity of property, we illustrate distinct application scenarios by comparing an apartment in an urban area (Figure \ref{fig:case-2}) and an apartment in a rural area (Figure \ref{fig:case-1}).
Despite both properties being apartments, disparities in location contribute to differences in property density. 
The neighbors to the property in the urban area are closer to the property, and the number of neighbors is greater compared to the rural area.

Another potential use case involves factors that may influence house prices but are not included as input features in the model. 
By designing the property configuration as a range rather than a fixed number, users can incorporate more subjective thought into their inputs.
For instance, the layout of a property is also a crucial factor in determining its price.
A property with a well-designed layout, such as a founder pattern, may have a higher utilization rate in its area.
However, incorporating the layout factor directly into the model can be challenging.
By setting the upper bound of the building area in the property configuration as larger, our system can filter out neighboring properties that are slightly bigger than the target property.
This approach facilitates a more ideal imputation and valuation result, enhancing the accuracy of the predictions.

\begin{figure}
  \hfill
  \centering
  \begin{subfigure}{0.5\textwidth}
          \centering
          \includegraphics[width=\linewidth]{Figure/use_case_urbun.png}
          \caption{Apartment located in Taipei which is an urban area.}
          \label{fig:case-2}
  \end{subfigure}
  \par\bigskip
  \hfill
  \begin{subfigure}{0.5\textwidth}
          \centering
          \includegraphics[width=\linewidth]{Figure/use_case_country.png}
          \caption{Apartment located in Nantou which is a rural area.}
          \label{fig:case-1}
  \end{subfigure}
  \caption{Two Use Case Studies. The left side displays the location of the target property on the map. On the right side, the red frame shows the predicted price of the target property, the blue frame shows the feature after imputation, and the black frame shows the explanation of the results.}\label{fig:case-studies}
\end{figure}

==> Table/imputation.tex <==
\begin{tabular}{c|ccc}
 \toprule
  & Building & Apartment & House \\
 \midrule
 No Imputation & 35.8 & 21.44 & 26.24 \\
 % Default Imputation & 22.25 & 15.80 & 20.92 \\
 Average Imputation & 28.3 & 24.81 & 40.42 \\
 Ours & \textbf{22.29} & \textbf{15.82} & \textbf{20.26} \\
 \midrule
 \midrule
 Ideal Situation & 16.71 & 13.88 & 18.28 \\
 \bottomrule
\end{tabular}
